Learnable Spatial-Temporal Positional Encoding for Link Prediction

Accurate predictions rely on the expressiveness power of graph deep learning frameworks like graph neural networks and graph transformers, where a positional encoding mechanism has become much more indispensable in recent state-of-the-art works to record the canonical position information. However, the current positional encoding is limited in three aspects: (1) most positional encoding methods use pre-defined, and fixed functions, which are inadequate to adapt to the complex attributed graphs; (2) a few pioneering works proposed the learnable positional encoding but are still limited to the structural information, not considering the real-world time-evolving topological and feature information; (3) most positional encoding methods are equipped with transformers' attention mechanism to fully leverage their capabilities, where the dense or relational attention is often unaffordable on large-scale structured data. Hence, we aim to develop Learnable Spatial-Temporal Positional Encoding in an effective and efficient manner and propose a simple temporal link prediction model named L-STEP. Briefly, for L-STEP, we (1) prove the proposed positional learning scheme can preserve the graph property from the spatial-temporal spectral viewpoint, (2) verify that MLPs can fully exploit the expressiveness and reach transformers' performance on that encoding, (3) change different initial positional encoding inputs to show robustness, (4) analyze the theoretical complexity and obtain less empirical running time than SOTA, and (5) demonstrate its temporal link prediction out-performance on 13 classic datasets and with 10 algorithms in both transductive and inductive settings using 3 different sampling strategies. Also, L-STEP obtains the leading performance in the newest large-scale TGB benchmark. Our code is available at https://github.com/kthrn22/L-STEP.

==> tables/ablation_study_2.tex <==
% \begin{table}[!htbp]
% \centering
% \caption{Comparison between only LPE and \name\ with random negative sampling strategy}
% \resizebox{1.01\textwidth}{!}
% {
% \setlength{\tabcolsep}{0.9mm}
% {
% \begin{tabular}{c|cccc|cccc}
% \hline
%                           & \multicolumn{4}{c|}{Transductive setting}                                                                                                    & \multicolumn{4}{c}{Inductive setting}                                                                                                                               \\ \cline{2-9} 
%                           & \multicolumn{2}{c|}{AP}                                                    & \multicolumn{2}{c|}{ROC-AUC}                                    & \multicolumn{2}{c|}{AP}                                                                            & \multicolumn{2}{c}{ROC-AUC}                                    \\ \cline{2-9} 
% \multirow{-3}{*}{Dataset} & \name (OURS)              & \multicolumn{1}{c|}{Only LPE}                  & {\color[HTML]{1F1F1F} \name (OURS)} & Only LPE                  & {\color[HTML]{1F1F1F} \name (OURS)} & \multicolumn{1}{c|}{Only LPE}                                & {\color[HTML]{1F1F1F} \name (OURS)} & Only LPE                 \\ \hline
% Wikipedia                 & \textbf{99.34 $\pm$ 0.04} & \multicolumn{1}{c|}{99.07 $\pm$ 0.03}          & \textbf{99.48 $\pm$ 0.03}           & 99.42 $\pm$ 0.03          & \textbf{99.15 $\pm$ 0.04}           & \multicolumn{1}{c|}{98.77 $\pm$ 0.05}                        & \textbf{99.30 $\pm$ 0.03}           & 98.99$\pm$ 0.03          \\
% Reddit                    & \textbf{99.37 $\pm$ 0.04} & \multicolumn{1}{c|}{98.67 $\pm$ 0.07}          & \textbf{99.49 $\pm$ 0.03}           & 99.13 $\pm$ 0.05          & \textbf{98.02 $\pm$ 0.09}           & \multicolumn{1}{c|}{{\color[HTML]{1F1F1F} 95.44 $\pm$ 0.29}} & \textbf{98.49 $\pm$ 0.06}           & 96.71$\pm$0.16           \\
% MOOC                      & \textbf{86.94 $\pm$ 0.34} & \multicolumn{1}{c|}{81.55 $\pm$ 0.53}          & \textbf{89.28 $\pm$ 0.28}           & 83.04 $\pm$ 0.44          & \textbf{88.49 $\pm$ 0.24}           & \multicolumn{1}{c|}{80.04 $\pm$ 0.40}                        & \textbf{90.63 $\pm$ 0.21}           & 81.70$\pm$ 0.39          \\
% Lastfm                    & \textbf{96.06 $\pm$ 0.30} & \multicolumn{1}{c|}{92.84 $\pm$ 0.54}          & \textbf{97.52 $\pm$ 0.17}           & 94.43 $\pm$ 0.38          & \textbf{96.25 $\pm$ 0.43}           & \multicolumn{1}{c|}{94.27 $\pm$ 0.36}                        & \textbf{97.66 $\pm$ 0.21}           & 96.22$\pm$ 0.22          \\
% Enron                     & \textbf{93.96 $\pm$ 0.36} & \multicolumn{1}{c|}{93.82 $\pm$ 0.44}          & \textbf{95.98 $\pm$ 0.23}           & 95.95 $\pm$ 0.31          & \textbf{89.17 $\pm$ 0.88}           & \multicolumn{1}{c|}{89.15 $\pm$1.32}                         & 92.30 $\pm$ 0.57                    & \textbf{92.33 $\pm$0.79} \\
% Social Evo.               & \textbf{92.22 $\pm$ 0.25} & \multicolumn{1}{c|}{91.56 $\pm$ 0.79}          & \textbf{94.33 $\pm$ 0.21}           & 93.76 $\pm$ 0.63          & \textbf{91.71 $\pm$ 0.32}           & \multicolumn{1}{c|}{90.42$\pm$ 1.68}                         & \textbf{94.09 $\pm$ 0.24}           & 93.28$\pm$ 0.97          \\
% UCI                       & 96.67 $\pm$ 0.47          & \multicolumn{1}{c|}{\textbf{96.83 $\pm$ 0.19}} & 97.62 $\pm$ 0.23                    & \textbf{97.89 $\pm$ 0.10} & \textbf{94.60 $\pm$ 0.41}           & \multicolumn{1}{c|}{94.60 $\pm$ 0.46}                        & 95.88 $\pm$ 0.17                    & \textbf{96.17 $\pm$0.22} \\ \hline
% \end{tabular}
% }
% }
% \label{tab:ablation_study_1}
% \end{table}




% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[!htbp]
\centering
\caption{Comparison between only using LPE and \name\ on with random negative sampling strategy}
\resizebox{1.01\textwidth}{!}
{
\setlength{\tabcolsep}{0.9mm}
{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{c|cccc|cccc}
\hline
\multirow{3}{*}{Dataset} & \multicolumn{4}{c|}{Transductive setting}                                                                                          & \multicolumn{4}{c}{Inductive setting}                                                                                            \\ \cline{2-9} 
                         & \multicolumn{2}{c|}{AP}                                                    & \multicolumn{2}{c|}{ROC-AUC}                          & \multicolumn{2}{c|}{AP}                                                   & \multicolumn{2}{c}{ROC-AUC}                          \\ \cline{2-9} 
                         & \name (OURS)              & \multicolumn{1}{c|}{Only LPE}                  & \name (OURS)              & Only LPE                  & \name (OURS)              & \multicolumn{1}{c|}{Only LPE}                 & \name (OURS)              & Only LPE                 \\ \hline
Flights                  & 98.94 $\pm$ 0.10          & \multicolumn{1}{c|}{\textbf{99.10 $\pm$ 0.03}} & 99.38 $\pm$ 0.04          & \textbf{99.43 $\pm$ 0.06} & 97.43 $\pm$ 0.15          & \multicolumn{1}{c|}{\textbf{97.81 $\pm$0.25}} & 98.46 $\pm$ 0.07          & \textbf{98.62 $\pm$0.11} \\
Can. Parl.               & 98.24 $\pm$ 0.11          & \multicolumn{1}{c|}{\textbf{98.41 $\pm$ 0.06}} & 98.97 $\pm$ 0.06          & \textbf{99.03 $\pm$ 0.03} & \textbf{92.25$\pm$ 0.24}  & \multicolumn{1}{c|}{92.13 $\pm$ 0.24}         & 95.06 $\pm$ 0.11          & \textbf{95.09 $\pm$0.07} \\
US Legis.                & 76.74 $\pm$ 0.60          & \multicolumn{1}{c|}{\textbf{77.36 $\pm$ 0.26}} & 83.89 $\pm$ 0.43          & \textbf{84.36 $\pm$ 0.20} & 61.98 $\pm$ 1.31          & \multicolumn{1}{c|}{\textbf{63.47 $\pm$0.63}} & 66.18 $\pm$ 1.19          & \textbf{66.75$\pm$ 0.57} \\
UN Trade                 & 75.84 $\pm$ 2.08          & \multicolumn{1}{c|}{\textbf{78.46 $\pm$ 0.97}} & \textbf{83.17 $\pm$ 1.28} & 77.81 $\pm$ 1.78          & 76.80 $\pm$ 2.01          & \multicolumn{1}{c|}{\textbf{84.85$\pm$ 0.89}} & 83.95 $\pm$ 1.76          & \textbf{84.89$\pm$ 1.39} \\
UN Vote                  & \textbf{73.40 $\pm$ 0.03} & \multicolumn{1}{c|}{70.99 $\pm$ 0.11}          & \textbf{79.59 $\pm$ 0.02} & 76.67 $\pm$ 0.09          & \textbf{75.09 $\pm$ 0.34} & \multicolumn{1}{c|}{70.01$\pm$ 0.69}          & \textbf{82.01 $\pm$ 0.21} & 77.36 $\pm$0.51          \\
Contact                  & \textbf{98.16 $\pm$ 0.09} & \multicolumn{1}{c|}{97.73 $\pm$ 0.04}          & \textbf{98.72 $\pm$ 0.06} & 98.40 $\pm$ 0.03          & \textbf{97.25 $\pm$ 0.07} & \multicolumn{1}{c|}{96.38$\pm$ 0.09}          & \textbf{97.99 $\pm$ 0.07} & 97.37$\pm$ 0.07          \\ \hline
\end{tabular}
}
}
\label{tab:ablation_study_2}
\end{table}



==> tables/ap_inductive.tex <==
\begin{table}[!htbp]
\centering
\caption{AP for inductive dynamic link prediction with random, historical, and inductive negative sampling strategies.}
\resizebox{1.01\textwidth}{!}
{
\setlength{\tabcolsep}{0.9mm}
{
\begin{tabular}{c|c|ccccccccc}
\hline
NSS                    & Datasets    & JODIE        & DyRep        & TGAT         & TGN          & CAWN         & TCL          & GraphMixer   & DyGFormer    & TempGT\\ \hline
\multirow{14}{*}{rnd}  & Wikipedia   & 94.82 $\pm$ 0.20 & 92.43 $\pm$ 0.37 & 96.22 $\pm$ 0.07 & 97.83 $\pm$ 0.04 & \underline{98.24 $\pm$ 0.03} & 96.22 $\pm$ 0.17 & 96.65 $\pm$ 0.02 & \textbf{98.59 $\pm$ 0.03} & 98.77 $\pm$ 0.05 \\
                       & Reddit      & 96.50 $\pm$ 0.13 & 96.09 $\pm$ 0.11 & 97.09 $\pm$ 0.04 & 97.50 $\pm$ 0.07 & \underline{98.62 $\pm$ 0.01} & 94.09 $\pm$ 0.07 & 95.26 $\pm$ 0.02 & \textbf{98.84 $\pm$ 0.02} & 95.44 $\pm$ 0.29                  \\
                       & MOOC        & 79.63 $\pm$ 1.92 & 81.07 $\pm$ 0.44 & 85.50 $\pm$ 0.19 & \textbf{89.04 $\pm$ 1.17} & 81.42 $\pm$ 0.24 & 80.60 $\pm$ 0.22 & 81.41 $\pm$ 0.21 & \underline{86.96 $\pm$ 0.43} & 80.04 $\pm$ 0.40 \\
                       & LastFM      & 81.61 $\pm$ 3.82 & 83.02 $\pm$ 1.48 & 78.63 $\pm$ 0.31 & 81.45 $\pm$ 4.29 & \underline{89.42 $\pm$ 0.07} & 73.53 $\pm$ 1.66 & 82.11 $\pm$ 0.42 & \textbf{94.23 $\pm$ 0.09} & 94.27 $\pm$ 0.36 \\
                       & Enron       & 80.72 $\pm$ 1.39 & 74.55 $\pm$ 3.95 & 67.05 $\pm$ 1.51 & 77.94 $\pm$ 1.02 & \underline{86.35 $\pm$ 0.51} & 76.14 $\pm$ 0.79 & 75.88 $\pm$ 0.48 & \textbf{89.76 $\pm$ 0.34} & 89.15 $\pm$ 1.32 \\
                       & Social Evo. & \underline{91.96 $\pm$ 0.48} & 90.04 $\pm$ 0.47 & 91.41 $\pm$ 0.16 & 90.77 $\pm$ 0.86 & 79.94 $\pm$ 0.18 & 91.55 $\pm$ 0.09 & 91.86 $\pm$ 0.06 & \textbf{93.14 $\pm$ 0.04} & 90.42 $\pm$ 1.68                  \\
                       & UCI         & 79.86 $\pm$ 1.48 & 57.48 $\pm$ 1.87 & 79.54 $\pm$ 0.48 & 88.12 $\pm$ 2.05 & \underline{92.73 $\pm$ 0.06} & 87.36 $\pm$ 2.03 & 91.19 $\pm$ 0.42 & \textbf{94.54 $\pm$ 0.12} & 94.60 $\pm$ 0.46 \\
                       & Flights     & 94.74 $\pm$ 0.37 & 92.88 $\pm$ 0.73 & 88.73 $\pm$ 0.33 & 95.03 $\pm$ 0.60 & \underline{97.06 $\pm$ 0.02} & 83.41 $\pm$ 0.07 & 83.03 $\pm$ 0.05 & \textbf{97.79 $\pm$ 0.02} & 97.81 $\pm$ 0.25                  \\
                       & Can. Parl.  & 53.92 $\pm$ 0.94 & 54.02 $\pm$ 0.76 & 55.18 $\pm$ 0.79 & 54.10 $\pm$ 0.93 & 55.80 $\pm$ 0.69 & 54.30 $\pm$ 0.66 & \underline{55.91 $\pm$ 0.82} & \textbf{87.74 $\pm$ 0.71} & 92.13 $\pm$ 0.24 \\
                       & US Legis.   & 54.93 $\pm$ 2.29 & \underline{57.28 $\pm$ 0.71} & 51.00 $\pm$ 3.11 & \textbf{58.63 $\pm$ 0.37} & 53.17 $\pm$ 1.20 & 52.59 $\pm$ 0.97 & 50.71 $\pm$ 0.76 & 54.28 $\pm$ 2.87 & 63.47 $\pm$ 0.63 \\
                       & UN Trade    & 59.65 $\pm$ 0.77 & 57.02 $\pm$ 0.69 & 61.03 $\pm$ 0.18 & 58.31 $\pm$ 3.15 & \textbf{65.24 $\pm$ 0.21} & 62.21 $\pm$ 0.12 & 62.17 $\pm$ 0.31 & \underline{64.55 $\pm$ 0.62} & 84.85 $\pm$ 0.89 \\
                       & UN Vote     & \underline{56.64 $\pm$ 0.96} & 54.62 $\pm$ 2.22 & 52.24 $\pm$ 1.46 & \textbf{58.85 $\pm$ 2.51} & 49.94 $\pm$ 0.45 & 51.60 $\pm$ 0.97 & 50.68 $\pm$ 0.44 & 55.93 $\pm$ 0.39 & 70.01 $\pm$ 0.69 \\
                       & Contact     & 94.34 $\pm$ 1.45 & 92.18 $\pm$ 0.41 & \underline{95.87 $\pm$ 0.11} & 93.82 $\pm$ 0.99 & 89.55 $\pm$ 0.30 & 91.11 $\pm$ 0.12 & 90.59 $\pm$ 0.05 & \textbf{98.03 $\pm$ 0.02} & 96.38 $\pm$ 0.09 \\ \cline{2-10} 
                       & Avg. Rank   & 4.69         & 5.77         & 5.23         & \underline{3.77}         & \underline{3.77}         & 5.77         & 5.23         & \textbf{1.54}         &  \\ \hline
\multirow{14}{*}{hist} & Wikipedia   & 68.69 $\pm$ 0.39 & 62.18 $\pm$ 1.27 & \underline{84.17 $\pm$ 0.22} & 81.76 $\pm$ 0.32 & 67.27 $\pm$ 1.63 & 82.20 $\pm$ 2.18 & \textbf{87.60 $\pm$ 0.30} & 71.42 $\pm$ 4.43 & 95.55 $\pm$ 0.22 \\
                       & Reddit      & 62.34 $\pm$ 0.54 & 61.60 $\pm$ 0.72 & 63.47 $\pm$ 0.36 & \underline{64.85 $\pm$ 0.85} & 63.67 $\pm$ 0.41 & 60.83 $\pm$ 0.25 & 64.50 $\pm$ 0.26 & \textbf{65.37 $\pm$ 0.60} &  \\
                       & MOOC        & 63.22 $\pm$ 1.55 & 62.93 $\pm$ 1.24 & 76.73 $\pm$ 0.29 & \underline{77.07 $\pm$ 3.41} & 74.68 $\pm$ 0.68 & 74.27 $\pm$ 0.53 & 74.00 $\pm$ 0.97 & \textbf{80.82 $\pm$ 0.30} &  \\
                       & LastFM      & 70.39 $\pm$ 4.31 & 71.45 $\pm$ 1.76 & 76.27 $\pm$ 0.25 & 66.65 $\pm$ 6.11 & 71.33 $\pm$ 0.47 & 65.78 $\pm$ 0.65 & \textbf{76.42 $\pm$ 0.22} & \underline{76.35 $\pm$ 0.52} & 89.66 $\pm$ 0.32  \\
                       & Enron       & 65.86 $\pm$ 3.71 & 62.08 $\pm$ 2.27 & 61.40 $\pm$ 1.31 & 62.91 $\pm$ 1.16 & 60.70 $\pm$ 0.36 & \underline{67.11 $\pm$ 0.62} & \textbf{72.37 $\pm$ 1.37} & 67.07 $\pm$ 0.62 &  \\
                       & Social Evo. & 88.51 $\pm$ 0.87 & 88.72 $\pm$ 1.10 & 93.97 $\pm$ 0.54 & 90.66 $\pm$ 1.62 & 79.83 $\pm$ 0.38 & \underline{94.10 $\pm$ 0.31} & 94.01 $\pm$ 0.47 & \textbf{96.82 $\pm$ 0.16} &  \\
                       & UCI         & 63.11 $\pm$ 2.27 & 52.47 $\pm$ 2.06 & 70.52 $\pm$ 0.93 & 70.78 $\pm$ 0.78 & 64.54 $\pm$ 0.47 & \underline{76.71 $\pm$ 1.00} & \textbf{81.66 $\pm$ 0.49} & 72.13 $\pm$ 1.87 & 85.54 $\pm$ 0.58 \\
                       & Flights     & 61.01 $\pm$ 1.65 & 62.83 $\pm$ 1.31 & \underline{64.72 $\pm$ 0.36} & 59.31 $\pm$ 1.43 & 56.82 $\pm$ 0.57 & 64.50 $\pm$ 0.25 & \textbf{65.28 $\pm$ 0.24} & 57.11 $\pm$ 0.21 &                  \\
                       & Can. Parl.  & 52.60 $\pm$ 0.88 & 52.28 $\pm$ 0.31 & 56.72 $\pm$ 0.47 & 54.42 $\pm$ 0.77 & \underline{57.14 $\pm$ 0.07} & 55.71 $\pm$ 0.74 & 55.84 $\pm$ 0.73 & \textbf{87.40 $\pm$ 0.85} & 72.01 $\pm$ 1.30 \\
                       & US Legis.   & 52.94 $\pm$ 2.11 & \textbf{62.10 $\pm$ 1.41} & 51.83 $\pm$ 3.95 & \underline{61.18 $\pm$ 1.10} & 55.56 $\pm$ 1.71 & 53.87 $\pm$ 1.41 & 52.03 $\pm$ 1.02 & 56.31 $\pm$ 3.46 & 64.67 $\pm$ 0.64 \\
                       & UN Trade    & 55.46 $\pm$ 1.19 & \underline{55.49 $\pm$ 0.84} & 55.28 $\pm$ 0.71 & 52.80 $\pm$ 3.19 & 55.00 $\pm$ 0.38 & \textbf{55.76 $\pm$ 1.03} & 54.94 $\pm$ 0.97 & 53.20 $\pm$ 1.07 & 76.57 $\pm$ 0.87 \\
                       & UN Vote     & \underline{61.04 $\pm$ 1.30} & 60.22 $\pm$ 1.78 & 53.05 $\pm$ 3.10 & \textbf{63.74 $\pm$ 3.00} & 47.98 $\pm$ 0.84 & 54.19 $\pm$ 2.17 & 48.09 $\pm$ 0.43 & 52.63 $\pm$ 1.26 & 72.20 $\pm$ 0.23 \\
                       & Contact     & 90.42 $\pm$ 2.34 & 89.22 $\pm$ 0.66 & \textbf{94.15 $\pm$ 0.45} & 88.13 $\pm$ 1.50 & 74.20 $\pm$ 0.80 & 90.44 $\pm$ 0.17 & 89.91 $\pm$ 0.36 & \underline{93.56 $\pm$ 0.52} &  \\ \cline{2-10} 
                       & Avg. Rank   & 5.38         & 5.46         & 4.00         & 4.54         & 5.92         & 3.92         & \underline{3.54}         & \textbf{3.23}         &  \\ \hline
\multirow{14}{*}{ind}  & Wikipedia   & 68.70 $\pm$ 0.39 & 62.19 $\pm$ 1.28 & \underline{84.17 $\pm$ 0.22} & 81.77 $\pm$ 0.32 & 67.24 $\pm$ 1.63 & 82.20 $\pm$ 2.18 & \textbf{87.60 $\pm$ 0.29} & 71.42 $\pm$ 4.43 & 95.56 ± 0.22 \\
                       & Reddit      & 62.32 $\pm$ 0.54 & 61.58 $\pm$ 0.72 & 63.40 $\pm$ 0.36 & \underline{64.84 $\pm$ 0.84} & 63.65 $\pm$ 0.41 & 60.81 $\pm$ 0.26 & 64.49 $\pm$ 0.25 & \textbf{65.35 $\pm$ 0.60} &  \\
                       & MOOC        & 63.22 $\pm$ 1.55 & 62.92 $\pm$ 1.24 & 76.72 $\pm$ 0.30 & \underline{77.07 $\pm$ 3.40} & 74.69 $\pm$ 0.68 & 74.28 $\pm$ 0.53 & 73.99 $\pm$ 0.97 & \textbf{80.82 $\pm$ 0.30} &  \\
                       & LastFM      & 70.39 $\pm$ 4.31 & 71.45 $\pm$ 1.75 & 76.28 $\pm$ 0.25 & 69.46 $\pm$ 4.65 & 71.33 $\pm$ 0.47 & 65.78 $\pm$ 0.65 & \textbf{76.42 $\pm$ 0.22} & \underline{76.35 $\pm$ 0.52} & 89.67 $\pm$ 0.32 \\
                       & Enron       & 65.86 $\pm$ 3.71 & 62.08 $\pm$ 2.27 & 61.40 $\pm$ 1.30 & 62.90 $\pm$ 1.16 & 60.72 $\pm$ 0.36 & \underline{67.11 $\pm$ 0.62} & \textbf{72.37 $\pm$ 1.38} & 67.07 $\pm$ 0.62 &  \\
                       & Social Evo. & 88.51 $\pm$ 0.87 & 88.72 $\pm$ 1.10 & 93.97 $\pm$ 0.54 & 90.65 $\pm$ 1.62 & 79.83 $\pm$ 0.39 & \underline{94.10 $\pm$ 0.32} & 94.01 $\pm$ 0.47 & \textbf{96.82 $\pm$ 0.17} &  \\
                       & UCI         & 63.16 $\pm$ 2.27 & 52.47 $\pm$ 2.09 & 70.49 $\pm$ 0.93 & 70.73 $\pm$ 0.79 & 64.54 $\pm$ 0.47 & \underline{76.65 $\pm$ 0.99} & \textbf{81.64 $\pm$ 0.49} & 72.13 $\pm$ 1.86 & 85.63 $\pm$ 0.59 \\
                       & Flights     & 61.01 $\pm$ 1.66 & 62.83 $\pm$ 1.31 & \underline{64.72 $\pm$ 0.37} & 59.32 $\pm$ 1.45 & 56.82 $\pm$ 0.56 & 64.50 $\pm$ 0.25 & \textbf{65.29 $\pm$ 0.24} & 57.11 $\pm$ 0.20 &  \\
                       & Can. Parl.  & 52.58 $\pm$ 0.86 & 52.24 $\pm$ 0.28 & 56.46 $\pm$ 0.50 & 54.18 $\pm$ 0.73 & \underline{57.06 $\pm$ 0.08} & 55.46 $\pm$ 0.69 & 55.76 $\pm$ 0.65 & \textbf{87.22 $\pm$ 0.82} & 71.81 $\pm$ 1.50 \\
                       & US Legis.   & 52.94 $\pm$ 2.11 & \textbf{62.10 $\pm$ 1.41} & 51.83 $\pm$ 3.95 & \underline{61.18 $\pm$ 1.10} & 55.56 $\pm$ 1.71 & 53.87 $\pm$ 1.41 & 52.03 $\pm$ 1.02 & 56.31 $\pm$ 3.46 & 64.67 $\pm$ 0.64 \\
                       & UN Trade    & 55.43 $\pm$ 1.20 & 55.42 $\pm$ 0.87 & \underline{55.58 $\pm$ 0.68} & 52.80 $\pm$ 3.24 & 54.97 $\pm$ 0.38 & \textbf{55.66 $\pm$ 0.98} & 54.88 $\pm$ 1.01 & 52.56 $\pm$ 1.70 & 76.56 ± 0.91 \\
                       & UN Vote     & \underline{61.17 $\pm$ 1.33} & 60.29 $\pm$ 1.79 & 53.08 $\pm$ 3.10 & \textbf{63.71 $\pm$ 2.97} & 48.01 $\pm$ 0.82 & 54.13 $\pm$ 2.16 & 48.10 $\pm$ 0.40 & 52.61 $\pm$ 1.25 &  72.23 $\pm$ 0.26\\
                       & Contact     & 90.43 $\pm$ 2.33 & 89.22 $\pm$ 0.65 & \textbf{94.14 $\pm$ 0.45} & 88.12 $\pm$ 1.50 & 74.19 $\pm$ 0.81 & 90.43 $\pm$ 0.17 & 89.91 $\pm$ 0.36 & \underline{93.55 $\pm$ 0.52} &  \\ \cline{2-10} 
                       & Avg. Rank   & 5.31         & 5.54         & 3.85         & 4.38         & 5.85         & 3.92         & \underline{3.46}         & \textbf{3.31}         &  \\ \hline
\end{tabular}
}
}
\label{tab:ap_inductive_dynamic_link_prediction}
\end{table}


==> tables/ap_transductive.tex <==



\begin{table}[!htbp]
\centering
\caption{AP for transductive dynamic link prediction with random, historical, and inductive negative sampling strategies. NSS is the abbreviation of Negative Sampling Strategies.}
\resizebox{1.01\textwidth}{!}
{
\setlength{\tabcolsep}{0.9mm}
{
\begin{tabular}{c|c|ccccccccc}
\hline
NSS                    & Datasets    & JODIE        & DyRep        & TGAT         & TGN          & CAWN     & TCL          & GraphMixer   & DyGFormer   & TempGT \\ \hline
\multirow{14}{*}{rnd}  & Wikipedia   & 96.50 $\pm$ 0.14 & 94.86 $\pm$ 0.06 & 96.94 $\pm$ 0.06 & 98.45 $\pm$ 0.06 & \underline{98.76 $\pm$ 0.03} & 96.47 $\pm$ 0.16 & 97.25 $\pm$ 0.03 & \textbf{99.03 $\pm$ 0.02} & \first{99.07 $\pm$ 0.03} \\
& Reddit      & 98.31 $\pm$ 0.14 & 98.22 $\pm$ 0.04 & 98.52 $\pm$ 0.02 & 98.63 $\pm$ 0.06 & \underline{99.11 $\pm$ 0.01} & 97.53 $\pm$ 0.02 & 97.31 $\pm$ 0.01 & \textbf{99.22 $\pm$ 0.01} & 98.67 $\pm$ 0.07 \\
& MOOC        & 80.23 $\pm$ 2.44 & 81.97 $\pm$ 0.49 & 85.84 $\pm$ 0.15 & \textbf{89.15 $\pm$ 1.60} & 80.15 $\pm$ 0.25 & 82.38 $\pm$ 0.24 & 82.78 $\pm$ 0.15 & \underline{87.52 $\pm$ 0.49} & 81.55 $\pm$ 0.53 \\
& LastFM      & 70.85 $\pm$ 2.13 & 71.92 $\pm$ 2.21 & 73.42 $\pm$ 0.21 & 77.07 $\pm$ 3.97 & \underline{86.99 $\pm$ 0.06} & 67.27 $\pm$ 2.16 & 75.61 $\pm$ 0.24 & \textbf{93.00 $\pm$ 0.12} & 92.84 $\pm$ 0.54 \\
& Enron       & 84.77 $\pm$ 0.30 & 82.38 $\pm$ 3.36 & 71.12 $\pm$ 0.97 & 86.53 $\pm$ 1.11 & \third{89.56 $\pm$ 0.09} & 79.70 $\pm$ 0.71 & 82.25 $\pm$ 0.16 & \second{92.47 $\pm$ 0.12} & \first{93.82 $\pm$ 0.44} \\
& Social Evo. & 89.89 $\pm$ 0.55 & 88.87 $\pm$ 0.30 & 93.16 $\pm$ 0.17 & \underline{93.57 $\pm$ 0.17} & 84.96 $\pm$ 0.09 & 93.13 $\pm$ 0.16 & 93.37 $\pm$ 0.07 & \textbf{94.73 $\pm$ 0.01} & 91.56 $\pm$ 0.79 \\
& UCI         & 89.43 $\pm$ 1.09 & 65.14 $\pm$ 2.30 & 79.63 $\pm$ 0.70 & 92.34 $\pm$ 1.04 & \underline{95.18 $\pm$ 0.06} & 89.57 $\pm$ 1.63 & 93.25 $\pm$ 0.57 & \textbf{95.79 $\pm$ 0.17} &  \first{96.83 $\pm$ 0.19} \\
& Flights     & 95.60 $\pm$ 1.73 & 95.29 $\pm$ 0.72 & 94.03 $\pm$ 0.18 & 97.95 $\pm$ 0.14 & \underline{98.51 $\pm$ 0.01} & 91.23 $\pm$ 0.02 & 90.99 $\pm$ 0.05 & \textbf{98.91 $\pm$ 0.01} & 99.10 $\pm$ 0.03 \\
& Can. Parl.  & 69.26 $\pm$ 0.31 & 66.54 $\pm$ 2.76 & 70.73 $\pm$ 0.72 & 70.88 $\pm$ 2.34 & 69.82 $\pm$ 2.34 & 68.67 $\pm$ 2.67 & \underline{77.04 $\pm$ 0.46} & \textbf{97.36 $\pm$ 0.45} & \first{98.41 $\pm$ 0.06} \\ 
& US Legis.   & 75.05 $\pm$ 1.52 & \underline{75.34 $\pm$ 0.39} & 68.52 $\pm$ 3.16 & \textbf{75.99 $\pm$ 0.58} & 70.58 $\pm$ 0.48 & 69.59 $\pm$ 0.48 & 70.74 $\pm$ 1.02 & 71.11 $\pm$ 0.59 & \first{77.36 $\pm$ 0.26} \\
& UN Trade    & 64.94 $\pm$ 0.31 & 63.21 $\pm$ 0.93 & 61.47 $\pm$ 0.18 & 65.03 $\pm$ 1.37 & \underline{65.39 $\pm$ 0.12} & 62.21 $\pm$ 0.03 & 62.61 $\pm$ 0.27 & \textbf{66.46 $\pm$ 1.29} & \first{78.46 $\pm$ 0.97} \\
& UN Vote     & \underline{63.91 $\pm$ 0.81} & 62.81 $\pm$ 0.80 & 52.21 $\pm$ 0.98 & \textbf{65.72 $\pm$ 2.17} & 52.84 $\pm$ 0.10 & 51.90 $\pm$ 0.30 & 52.11 $\pm$ 0.16 & 55.55 $\pm$ 0.42 & \first{70.99 $\pm$ 0.11} \\
& Contact     & 95.31 $\pm$ 1.33 & 95.98 $\pm$ 0.15 & 96.28 $\pm$ 0.09 & \underline{96.89 $\pm$ 0.56} & 90.26 $\pm$ 0.28 & 92.44 $\pm$ 0.12 & 91.92 $\pm$ 0.03 & \textbf{98.29 $\pm$ 0.01} & 97.73 $\pm$ 0.04 \\ \cline{2-11} 
& Avg. Rank   & 5.08         & 5.85         & 5.69         & \underline{2.54}         & 4.31         & 6.92         & 5.46         & \textbf{1.62}         & \\ \hline

                       \multirow{14}{*}{hist} & Wikipedia   & 83.01 $\pm$ 0.66 & 79.93 $\pm$ 0.56 & 87.38 $\pm$ 0.22 & 86.86 $\pm$ 0.33 & 71.21 $\pm$ 1.67 & \underline{89.05 $\pm$ 0.39} & \textbf{90.90 $\pm$ 0.10} & 82.23 $\pm$ 2.54 & 97.65 $\pm$ 0.09 \\
                       & Reddit      & 80.03 $\pm$ 0.36 & 79.83 $\pm$ 0.31 & 79.55 $\pm$ 0.20 & \underline{81.22 $\pm$ 0.61} & 80.82 $\pm$ 0.45 & 77.14 $\pm$ 0.16 & 78.44 $\pm$ 0.18 & \textbf{81.57 $\pm$ 0.67} &  \\
                       & MOOC        & 78.94 $\pm$ 1.25 & 75.60 $\pm$ 1.12 & 82.19 $\pm$ 0.62 & \textbf{87.06 $\pm$ 1.93} & 74.05 $\pm$ 0.95 & 77.06 $\pm$ 0.41 & 77.77 $\pm$ 0.92 & \underline{85.85 $\pm$ 0.66} & \\
                       & LastFM      & 74.35 $\pm$ 3.81 & 74.92 $\pm$ 2.46 & 71.59 $\pm$ 0.24 & \underline{76.87 $\pm$ 4.64} & 69.86 $\pm$ 0.43 & 59.30 $\pm$ 2.31 & 72.47 $\pm$ 0.49 & \textbf{81.57 $\pm$ 0.48} & 91.96 $\pm$ 1.15 \\
                       & Enron       & 69.85 $\pm$ 2.70 & 71.19 $\pm$ 2.76 & 64.07 $\pm$ 1.05 & 73.91 $\pm$ 1.76 & 64.73 $\pm$ 0.36 & 70.66 $\pm$ 0.39 & \textbf{77.98 $\pm$ 0.92} & 75.63 $\pm$ 0.73 & \\
                       & Social Evo. & 87.44 $\pm$ 6.78 & 93.29 $\pm$ 0.43 & \underline{95.01 $\pm$ 0.44} & 94.45 $\pm$ 0.56 & 85.53 $\pm$ 0.38 & 94.74 $\pm$ 0.31 & 94.93 $\pm$ 0.31 & \textbf{97.38 $\pm$ 0.14} & \\
                       & UCI         & 75.24 $\pm$ 5.80 & 55.10 $\pm$ 3.14 & 68.27 $\pm$ 1.37 & 80.43 $\pm$ 2.12 & 65.30 $\pm$ 0.43 & 80.25 $\pm$ 2.74 & \textbf{84.11 $\pm$ 1.35} & \underline{82.17 $\pm$ 0.82} & 93.63 $\pm$ 0.33 \\
                       & Flights     & 66.48 $\pm$ 2.59 & 67.61 $\pm$ 0.99 & \textbf{72.38 $\pm$ 0.18} & 66.70 $\pm$ 1.64 & 64.72 $\pm$ 0.97 & 70.68 $\pm$ 0.24 & \underline{71.47 $\pm$ 0.26} & 66.59 $\pm$ 0.49 & \\
                       & Can. Parl.  & 51.79 $\pm$ 0.63 & 63.31 $\pm$ 1.23 & 67.13 $\pm$ 0.84 & 68.42 $\pm$ 3.07 & 66.53 $\pm$ 2.77 & 65.93 $\pm$ 3.00 & \underline{74.34 $\pm$ 0.87} & \textbf{97.00 $\pm$ 0.31} & 88.42 $\pm$ 2.46 \\
                       & US Legis.   & 51.71 $\pm$ 5.76 & \textbf{86.88 $\pm$ 2.25} & 62.14 $\pm$ 6.60 & 74.00 $\pm$ 7.57 & 68.82 $\pm$ 8.23 & 80.53 $\pm$ 3.95 & 81.65 $\pm$ 1.02 & \underline{85.30 $\pm$ 3.88} & 82.85 $\pm$ 1.90 \\
                       & UN Trade    & 61.39 $\pm$ 1.83 & 59.19 $\pm$ 1.07 & 55.74 $\pm$ 0.91 & 58.44 $\pm$ 5.51 & 55.71 $\pm$ 0.38 & 55.90 $\pm$ 1.17 & 57.05 $\pm$ 1.22 & \underline{64.41 $\pm$ 1.40} & 78.62 $\pm$ 0.98 \\
                       & UN Vote     & \underline{70.02 $\pm$ 0.81} & 69.30 $\pm$ 1.12 & 52.96 $\pm$ 2.14 & 69.37 $\pm$ 3.93 & 51.26 $\pm$ 0.04 & 52.30 $\pm$ 2.35 & 51.20 $\pm$ 1.60 & 60.84 $\pm$ 1.58 & 76.19 $\pm$ 0.16 \\
                       & Contact     & 95.31 $\pm$ 2.13 & \underline{96.39 $\pm$ 0.20} & 96.05 $\pm$ 0.52 & 93.05 $\pm$ 2.35 & 84.16 $\pm$ 0.49 & 93.86 $\pm$ 0.21 & 93.36 $\pm$ 0.41 & \textbf{97.57 $\pm$ 0.06} & \\ \cline{2-11} 
                       & Avg. Rank   & 5.46         & 5.08         & 5.08         & \underline{3.85}         & 7.54         & 5.46         & 4.00         & \textbf{2.62}          \\ \hline
\multirow{14}{*}{ind}  & Wikipedia   & 75.65 $\pm$ 0.79 & 70.21 $\pm$ 1.58 & \underline{87.00 $\pm$ 0.16} & 85.62 $\pm$ 0.44 & 74.06 $\pm$ 2.62 & 86.76 $\pm$ 0.72 & \textbf{88.59 $\pm$ 0.17} & 78.29 $\pm$ 5.38 & 94.97 ± 0.25\\
                       & Reddit      & 86.98 $\pm$ 0.16 & 86.30 $\pm$ 0.26 & 89.59 $\pm$ 0.24 & 88.10 $\pm$ 0.24 & \textbf{91.67 $\pm$ 0.24} & 87.45 $\pm$ 0.29 & 85.26 $\pm$ 0.11 & \underline{91.11 $\pm$ 0.40} & \\
                       & MOOC        & 65.23 $\pm$ 2.19 & 61.66 $\pm$ 0.95 & 75.95 $\pm$ 0.64 & \underline{77.50 $\pm$ 2.91} & 73.51 $\pm$ 0.94 & 74.65 $\pm$ 0.54 & 74.27 $\pm$ 0.92 & \textbf{81.24 $\pm$ 0.69} & \\
                       & LastFM      & 62.67 $\pm$ 4.49 & 64.41 $\pm$ 2.70 & 71.13 $\pm$ 0.17 & 65.95 $\pm$ 5.98 & 67.48 $\pm$ 0.77 & 58.21 $\pm$ 0.89 & 68.12 $\pm$ 0.33 & \underline{73.97 $\pm$ 0.50} & 89.72 $\pm$ 1.42 \\
                       & Enron       & 68.96 $\pm$ 0.98 & 67.79 $\pm$ 1.53 & 63.94 $\pm$ 1.36 & 70.89 $\pm$ 2.72 & \underline{75.15 $\pm$ 0.58} & 71.29 $\pm$ 0.32 & 75.01 $\pm$ 0.79 & \textbf{77.41 $\pm$ 0.89} & \\
                       & Social Evo. & 89.82 $\pm$ 4.11 & 93.28 $\pm$ 0.48 & 94.84 $\pm$ 0.44 & \underline{95.13 $\pm$ 0.56} & 88.32 $\pm$ 0.27 & 94.90 $\pm$ 0.36 & 94.72 $\pm$ 0.33 & \textbf{97.68 $\pm$ 0.10} & \\
                       & UCI         & 65.99 $\pm$ 1.40 & 54.79 $\pm$ 1.76 & 68.67 $\pm$ 0.84 & 70.94 $\pm$ 0.71 & 64.61 $\pm$ 0.48 & \underline{76.01 $\pm$ 1.11} & \textbf{80.10 $\pm$ 0.51} & 72.25 $\pm$ 1.71 & 83.71 $\pm$ 0.42 \\
                       & Flights     & 69.07 $\pm$ 4.02 & 70.57 $\pm$ 1.82 & \underline{75.48 $\pm$ 0.26} & 71.09 $\pm$ 2.72 & 69.18 $\pm$ 1.52 & 74.62 $\pm$ 0.18 & 74.87 $\pm$ 0.21 & 70.92 $\pm$ 1.78 & \\
                       & Can. Parl.  & 48.42 $\pm$ 0.66 & 58.61 $\pm$ 0.86 & 68.82 $\pm$ 1.21 & 65.34 $\pm$ 2.87 & 67.75 $\pm$ 1.00 & 65.85 $\pm$ 1.75 & \underline{69.48 $\pm$ 0.63} & \textbf{95.44 $\pm$ 0.57} & 81.72 $\pm$ 2.98 \\
                       & US Legis.   & 50.27 $\pm$ 5.13 & \textbf{83.44 $\pm$ 1.16} & 61.91 $\pm$ 5.82 & 67.57 $\pm$ 6.47 & 65.81 $\pm$ 8.52 & 78.15 $\pm$ 3.34 & 79.63 $\pm$ 0.84 & \underline{81.25 $\pm$ 3.62} & 77.23 $\pm$ 0.30 \\
                       & UN Trade    & 60.42 $\pm$ 1.48 & 60.19 $\pm$ 1.24 & 60.61 $\pm$ 1.24 & 61.04 $\pm$ 6.01 & \underline{62.54 $\pm$ 0.67} & 61.06 $\pm$ 1.74 & 60.15 $\pm$ 1.29 & 55.79 $\pm$ 1.02 & 78.51 ± 0.85 \\
                       & UN Vote     & \textbf{67.79 $\pm$ 1.46} & 67.53 $\pm$ 1.98 & 52.89 $\pm$ 1.61 & \underline{67.63 $\pm$ 2.67} & 52.19 $\pm$ 0.34 & 50.62 $\pm$ 0.82 & 51.60 $\pm$ 0.73 & 51.91 $\pm$ 0.84 & 73.34 $\pm$ 0.19 \\
                       & Contact     & 93.43 $\pm$ 1.78 & 94.18 $\pm$ 0.10 & \underline{94.35 $\pm$ 0.48} & 90.18 $\pm$ 3.28 & 89.31 $\pm$ 0.27 & 91.35 $\pm$ 0.21 & 90.87 $\pm$ 0.35 & \textbf{94.75 $\pm$ 0.28} & \\ \cline{2-11} 
                       & Avg. Rank   & 6.62         & 6.38         & \underline{4.15}         & 4.38         & 5.46         & 4.69         & 4.46         & \textbf{3.23}         &\\ \hline
\end{tabular}
}
}
\label{tab:average_precision_transductive_dynamic_link_prediction}
\end{table}

==> tables/auc_roc_inductive.tex <==


\begin{table}[!htbp]
\centering
\caption{AUC-ROC for inductive dynamic link prediction with random, historical, and inductive negative sampling strategies.}
\resizebox{1.01\textwidth}{!}
{
\setlength{\tabcolsep}{0.9mm}
{
\begin{tabular}{c|c|ccccccccc}
\hline
NSS                    & Datasets    & JODIE        & DyRep        & TGAT         & TGN          & CAWN         & TCL          & GraphMixer   & DyGFormer    & TempGT\\ \hline
\multirow{14}{*}{rnd}  & Wikipedia   & 94.33 $\pm$ 0.27 & 91.49 $\pm$ 0.45 & 95.90 $\pm$ 0.09 & 97.72 $\pm$ 0.03 & \underline{98.03 $\pm$ 0.04} & 95.57 $\pm$ 0.20 & 96.30 $\pm$ 0.04 & \textbf{98.48 $\pm$ 0.03} & 98.99 $\pm$ 0.03 \\
                       & Reddit      & 96.52 $\pm$ 0.13 & 96.05 $\pm$ 0.12 & 96.98 $\pm$ 0.04 & 97.39 $\pm$ 0.07 & \underline{98.42 $\pm$ 0.02} & 93.80 $\pm$ 0.07 & 94.97 $\pm$ 0.05 & \textbf{98.71 $\pm$ 0.01} & 96.71 $\pm$ 0.16 \\
                       & MOOC        & 83.16 $\pm$ 1.30 & 84.03 $\pm$ 0.49 & 86.84 $\pm$ 0.17 & \textbf{91.24 $\pm$ 0.99} & 81.86 $\pm$ 0.25 & 81.43 $\pm$ 0.19 & 82.77 $\pm$ 0.24 & \underline{87.62 $\pm$ 0.51} & 81.70 $\pm$ 0.39 \\
                       & LastFM      & 81.13 $\pm$ 3.39 & 82.24 $\pm$ 1.51 & 76.99 $\pm$ 0.29 & 82.61 $\pm$ 3.15 & \underline{87.82 $\pm$ 0.12} & 70.84 $\pm$ 0.85 & 80.37 $\pm$ 0.18 & \textbf{94.08 $\pm$ 0.08} & 96.22 $\pm$ 0.22 \\
                       & Enron       & 81.96 $\pm$ 1.34 & 76.34 $\pm$ 4.20 & 64.63 $\pm$ 1.74 & 78.83 $\pm$ 1.11 & \underline{87.02 $\pm$ 0.50} & 72.33 $\pm$ 0.99 & 76.51 $\pm$ 0.71 & \textbf{90.69 $\pm$ 0.26} & 92.33 $\pm$ 0.79 \\
                       & Social Evo. & 93.70 $\pm$ 0.29 & 91.18 $\pm$ 0.49 & 93.41 $\pm$ 0.19 & 93.43 $\pm$ 0.59 & 84.73 $\pm$ 0.27 & 93.71 $\pm$ 0.18 & \underline{94.09 $\pm$ 0.07} & \textbf{95.29 $\pm$ 0.03} & 93.28 $\pm$ 0.97  \\
                       & UCI         & 78.80 $\pm$ 0.94 & 58.08 $\pm$ 1.81 & 77.64 $\pm$ 0.38 & 86.68 $\pm$ 2.29 & \underline{90.40 $\pm$ 0.11} & 84.49 $\pm$ 1.82 & 89.30 $\pm$ 0.57 & \textbf{92.63 $\pm$ 0.13} & 96.17 $\pm$ 0.22 \\
                       & Flights     & 95.21 $\pm$ 0.32 & 93.56 $\pm$ 0.70 & 88.64 $\pm$ 0.35 & 95.92 $\pm$ 0.43 & \underline{96.86 $\pm$ 0.02} & 82.48 $\pm$ 0.01 & 82.27 $\pm$ 0.06 & \textbf{97.80 $\pm$ 0.02} & 98.62 $\pm$ 0.11  \\
                       & Can. Parl.  & 53.81 $\pm$ 1.14 & 55.27 $\pm$ 0.49 & 56.51 $\pm$ 0.75 & 55.86 $\pm$ 0.75 & \underline{58.83 $\pm$ 1.13} & 55.83 $\pm$ 1.07 & 58.32 $\pm$ 1.08 & \textbf{89.33 $\pm$ 0.48} & 95.09 $\pm$ 0.07 \\
                       & US Legis.   & 58.12 $\pm$ 2.35 & \underline{61.07 $\pm$ 0.56} & 48.27 $\pm$ 3.50 & \textbf{62.38 $\pm$ 0.48} & 51.49 $\pm$ 1.13 & 50.43 $\pm$ 1.48 & 47.20 $\pm$ 0.89 & 53.21 $\pm$ 3.04 & 66.75 $\pm$ 0.57 \\
                       & UN Trade    & 62.28 $\pm$ 0.50 & 58.82 $\pm$ 0.98 & 62.72 $\pm$ 0.12 & 59.99 $\pm$ 3.50 & \underline{67.05 $\pm$ 0.21} & 63.76 $\pm$ 0.07 & 63.48 $\pm$ 0.37 & \textbf{67.25 $\pm$ 1.05} & 84.89 $\pm$ 1.39 \\
                       & UN Vote     & \underline{58.13 $\pm$ 1.43} & 55.13 $\pm$ 3.46 & 51.83 $\pm$ 1.35 & \textbf{61.23 $\pm$ 2.71} & 48.34 $\pm$ 0.76 & 50.51 $\pm$ 1.05 & 50.04 $\pm$ 0.86 & 56.73 $\pm$ 0.69 & 77.36 $\pm$ 0.51  \\
                       & Contact     & 95.37 $\pm$ 0.92 & 91.89 $\pm$ 0.38 & \underline{96.53 $\pm$ 0.10} & 94.84 $\pm$ 0.75 & 89.07 $\pm$ 0.34 & 93.05 $\pm$ 0.09 & 92.83 $\pm$ 0.05 & \textbf{98.30 $\pm$ 0.02} & 97.37 $\pm$ 0.07  \\ \cline{2-10} 
                       & Avg. Rank   & 4.69         & 5.85         & 5.31         & \underline{3.38}         & 4.00         & 6.00         & 5.31         & \textbf{1.46}         &  \\ \hline
\multirow{14}{*}{hist} & Wikipedia   & 61.86 $\pm$ 0.53 & 57.54 $\pm$ 1.09 & 78.38 $\pm$ 0.20 & 75.75 $\pm$ 0.29 & 62.04 $\pm$ 0.65 & \underline{79.79 $\pm$ 0.96} & \textbf{82.87 $\pm$ 0.21} & 68.33 $\pm$ 2.82 & 96.31 $\pm$ 0.14 \\
                       & Reddit      & 61.69 $\pm$ 0.39 & 60.45 $\pm$ 0.37 & 64.43 $\pm$ 0.27 & 64.55 $\pm$ 0.50 & \textbf{64.94 $\pm$ 0.21} & 61.43 $\pm$ 0.26 & 64.27 $\pm$ 0.13 & \underline{64.81 $\pm$ 0.25} &  \\
                       & MOOC        & 64.48 $\pm$ 1.64 & 64.23 $\pm$ 1.29 & 74.08 $\pm$ 0.27 & \underline{77.69 $\pm$ 3.55} & 71.68 $\pm$ 0.94 & 69.82 $\pm$ 0.32 & 72.53 $\pm$ 0.84 & \textbf{80.77 $\pm$ 0.63} &  \\
                       & LastFM      & 68.44 $\pm$ 3.26 & 68.79 $\pm$ 1.08 & 69.89 $\pm$ 0.28 & 66.99 $\pm$ 5.62 & 67.69 $\pm$ 0.24 & 55.88 $\pm$ 1.85 & \underline{70.07 $\pm$ 0.20} & \textbf{70.73 $\pm$ 0.37} & 92.97 $\pm$ 0.25 \\
                       & Enron       & 65.32 $\pm$ 3.57 & 61.50 $\pm$ 2.50 & 57.84 $\pm$ 2.18 & 62.68 $\pm$ 1.09 & 62.25 $\pm$ 0.40 & 64.06 $\pm$ 1.02 & \textbf{68.20 $\pm$ 1.62} & \underline{65.78 $\pm$ 0.42} &  \\
                       & Social Evo. & 88.53 $\pm$ 0.55 & 87.93 $\pm$ 1.05 & 91.87 $\pm$ 0.72 & 92.10 $\pm$ 1.22 & 83.54 $\pm$ 0.24 & 93.28 $\pm$ 0.60 & \underline{93.62 $\pm$ 0.35} & \textbf{96.91 $\pm$ 0.09} &  \\
                       & UCI         & 60.24 $\pm$ 1.94 & 51.25 $\pm$ 2.37 & 62.32 $\pm$ 1.18 & 62.69 $\pm$ 0.90 & 56.39 $\pm$ 0.10 & \underline{70.46 $\pm$ 1.94} & \textbf{75.98 $\pm$ 0.84} & 65.55 $\pm$ 1.01 & 88.42 $\pm$ 0.40 \\
                       & Flights     & 60.72 $\pm$ 1.29 & 61.99 $\pm$ 1.39 & \underline{63.38 $\pm$ 0.26} & 59.66 $\pm$ 1.04 & 56.58 $\pm$ 0.44 & \textbf{63.48 $\pm$ 0.23} & 63.30 $\pm$ 0.19 & 56.05 $\pm$ 0.21 &  \\
                       & Can. Parl.  & 51.62 $\pm$ 1.00 & 52.38 $\pm$ 0.46 & 58.30 $\pm$ 0.61 & 55.64 $\pm$ 0.54 & \underline{60.11 $\pm$ 0.48} & 57.30 $\pm$ 1.03 & 56.68 $\pm$ 1.20 & \textbf{88.68 $\pm$ 0.74} & 78.92 $\pm$ 1.22 \\
                       & US Legis.   & 58.12 $\pm$ 2.94 & \textbf{67.94 $\pm$ 0.98} & 49.99 $\pm$ 4.88 & \underline{64.87 $\pm$ 1.65} & 54.41 $\pm$ 1.31 & 52.12 $\pm$ 2.13 & 49.28 $\pm$ 0.86 & 56.57 $\pm$ 3.22 & 67.74 $\pm$ 0.61 \\
                       & UN Trade    & 58.73 $\pm$ 1.19 & 57.90 $\pm$ 1.33 & 59.74 $\pm$ 0.59 & 55.61 $\pm$ 3.54 & \underline{60.95 $\pm$ 0.80} & \textbf{61.12 $\pm$ 0.97} & 59.88 $\pm$ 1.17 & 58.46 $\pm$ 1.65 & 82.47 $\pm$ 0.68  \\
                       & UN Vote     & \underline{65.16 $\pm$ 1.28} & 63.98 $\pm$ 2.12 & 51.73 $\pm$ 4.12 & \textbf{68.59 $\pm$ 3.11} & 48.01 $\pm$ 1.77 & 54.66 $\pm$ 2.11 & 45.49 $\pm$ 0.42 & 53.85 $\pm$ 2.02 & 78.30 $\pm$ 0.19 \\
                       & Contact     & 90.80 $\pm$ 1.18 & 88.88 $\pm$ 0.68 & \underline{93.76 $\pm$ 0.41} & 88.84 $\pm$ 1.39 & 74.79 $\pm$ 0.37 & 90.37 $\pm$ 0.16 & 90.04 $\pm$ 0.29 & \textbf{94.14 $\pm$ 0.26} &  \\ \cline{2-10} 
                       & Avg. Rank   & 5.08         & 6.00         & 4.23         & 4.54         & 5.38         & 4.00         & \underline{3.69}         & \textbf{3.08}         &  \\ \hline
\multirow{14}{*}{ind}  & Wikipedia   & 61.87 $\pm$ 0.53 & 57.54 $\pm$ 1.09 & 78.38 $\pm$ 0.20 & 75.76 $\pm$ 0.29 & 62.02 $\pm$ 0.65 & \underline{79.79 $\pm$ 0.96} & \textbf{82.88 $\pm$ 0.21} & 68.33 $\pm$ 2.82 & 96.32 ± 0.14 \\
                       & Reddit      & 61.69 $\pm$ 0.39 & 60.44 $\pm$ 0.37 & 64.39 $\pm$ 0.27 & 64.55 $\pm$ 0.50 & \textbf{64.91 $\pm$ 0.21} & 61.36 $\pm$ 0.26 & 64.27 $\pm$ 0.13 & \underline{64.80 $\pm$ 0.25} &  \\
                       & MOOC        & 64.48 $\pm$ 1.64 & 64.22 $\pm$ 1.29 & 74.07 $\pm$ 0.27 & \underline{77.68 $\pm$ 3.55} & 71.69 $\pm$ 0.94 & 69.83 $\pm$ 0.32 & 72.52 $\pm$ 0.84 & \textbf{80.77 $\pm$ 0.63} &  \\
                       & LastFM      & 68.44 $\pm$ 3.26 & 68.79 $\pm$ 1.08 & 69.89 $\pm$ 0.28 & 66.99 $\pm$ 5.61 & 67.68 $\pm$ 0.24 & 55.88 $\pm$ 1.85 & \underline{70.07 $\pm$ 0.20} & \textbf{70.73 $\pm$ 0.37} & 92.98 $\pm$ 0.25 \\
                       & Enron       & 65.32 $\pm$ 3.57 & 61.50 $\pm$ 2.50 & 57.83 $\pm$ 2.18 & 62.68 $\pm$ 1.09 & 62.27 $\pm$ 0.40 & 64.05 $\pm$ 1.02 & \textbf{68.19 $\pm$ 1.63} & \underline{65.79 $\pm$ 0.42} &  \\
                       & Social Evo. & 88.53 $\pm$ 0.55 & 87.93 $\pm$ 1.05 & 91.88 $\pm$ 0.72 & 92.10 $\pm$ 1.22 & 83.54 $\pm$ 0.24 & 93.28 $\pm$ 0.60 & \underline{93.62 $\pm$ 0.35} & \textbf{96.91 $\pm$ 0.09} &  \\
                       & UCI         & 60.27 $\pm$ 1.94 & 51.26 $\pm$ 2.40 & 62.29 $\pm$ 1.17 & 62.66 $\pm$ 0.91 & 56.39 $\pm$ 0.11 & \underline{70.42 $\pm$ 1.93} & \textbf{75.97 $\pm$ 0.85} & 65.58 $\pm$ 1.00 & 88.52 $\pm$ 0.39 \\
                       & Flights     & 60.72 $\pm$ 1.29 & 61.99 $\pm$ 1.39 & \underline{63.40 $\pm$ 0.26} & 59.66 $\pm$ 1.05 & 56.58 $\pm$ 0.44 & \textbf{63.49 $\pm$ 0.23} & 63.32 $\pm$ 0.19 & 56.05 $\pm$ 0.22 &  \\
                       & Can. Parl.  & 51.61 $\pm$ 0.98 & 52.35 $\pm$ 0.52 & 58.15 $\pm$ 0.62 & 55.43 $\pm$ 0.42 & \underline{60.01 $\pm$ 0.47} & 56.88 $\pm$ 0.93 & 56.63 $\pm$ 1.09 & \textbf{88.51 $\pm$ 0.73} & 78.63 $\pm$ 1.42 \\
                       & US Legis.   & 58.12 $\pm$ 2.94 & \textbf{67.94 $\pm$ 0.98} & 49.99 $\pm$ 4.88 & \underline{64.87 $\pm$ 1.65} & 54.41 $\pm$ 1.31 & 52.12 $\pm$ 2.13 & 49.28 $\pm$ 0.86 & 56.57 $\pm$ 3.22 & 67.74 $\pm$ 0.61 \\
                       & UN Trade    & 58.71 $\pm$ 1.20 & 57.87 $\pm$ 1.36 & 59.98 $\pm$ 0.59 & 55.62 $\pm$ 3.59 & \underline{60.88 $\pm$ 0.79} & \textbf{61.01 $\pm$ 0.93} & 59.71 $\pm$ 1.17 & 57.28 $\pm$ 3.06 & 82.48 ± 0.68 \\
                       & UN Vote     & \underline{65.29 $\pm$ 1.30} & 64.10 $\pm$ 2.10 & 51.78 $\pm$ 4.14 & \textbf{68.58 $\pm$ 3.08} & 48.04 $\pm$ 1.76 & 54.65 $\pm$ 2.20 & 45.57 $\pm$ 0.41 & 53.87 $\pm$ 2.01 & 78.31 $\pm$ 0.21  \\
                       & Contact     & 90.80 $\pm$ 1.18 & 88.87 $\pm$ 0.67 & \underline{93.76 $\pm$ 0.40} & 88.85 $\pm$ 1.39 & 74.79 $\pm$ 0.38 & 90.37 $\pm$ 0.16 & 90.04 $\pm$ 0.29 & \textbf{94.14 $\pm$ 0.26} &  \\ \cline{2-10} 
                       & Avg. Rank   & 5.08         & 5.92         & 4.15         & 4.54         & 5.38         & 4.00         & \underline{3.77}         & \textbf{3.15}         &  \\ \hline
\end{tabular}
}
}
\label{tab:auc_roc_inductive_dynamic_link_prediction}
\end{table}

==> tables/auc_roc_transductive.tex <==
\begin{table}[!htbp]
\centering
\caption{AUC-ROC for transductive dynamic link prediction with random, historical, and inductive negative sampling strategies.}
\resizebox{1.01\textwidth}{!}
{
\setlength{\tabcolsep}{0.9mm}
{
\begin{tabular}{c|c|ccccccccc}
\hline
NSS                    & Datasets    & JODIE        & DyRep        & TGAT         & TGN          & CAWN     & TCL          & GraphMixer   & DyGFormer    & TempGT\\ \hline
\multirow{14}{*}{rnd}  & Wikipedia   & 96.33 $\pm$ 0.07 & 94.37 $\pm$ 0.09 & 96.67 $\pm$ 0.07 & 98.37 $\pm$ 0.07 & \underline{98.54 $\pm$ 0.04} & 95.84 $\pm$ 0.18 & 96.92 $\pm$ 0.03 & \textbf{98.91 $\pm$ 0.02} & \first{99.42 $\pm$ 0.03} \\
                       & Reddit      & 98.31 $\pm$ 0.05 & 98.17 $\pm$ 0.05 & 98.47 $\pm$ 0.02 & 98.60 $\pm$ 0.06 & \underline{99.01 $\pm$ 0.01} & 97.42 $\pm$ 0.02 & 97.17 $\pm$ 0.02 & \textbf{99.15 $\pm$ 0.01} & 99.13 $\pm$ 0.05                 \\
                       & MOOC        & 83.81 $\pm$ 2.09 & 85.03 $\pm$ 0.58 & 87.11 $\pm$ 0.19 & \textbf{91.21 $\pm$ 1.15} & 80.38 $\pm$ 0.26 & 83.12 $\pm$ 0.18 & 84.01 $\pm$ 0.17 & \underline{87.91 $\pm$ 0.58} & 83.04 $\pm$ 0.44 \\
                       & LastFM      & 70.49 $\pm$ 1.66 & 71.16 $\pm$ 1.89 & 71.59 $\pm$ 0.18 & 78.47 $\pm$ 2.94 & \underline{85.92 $\pm$ 0.10} & 64.06 $\pm$ 1.16 & 73.53 $\pm$ 0.12 & \textbf{93.05 $\pm$ 0.10} & \first{94.43 $\pm$ 0.38} \\
                       & Enron       & 87.96 $\pm$ 0.52 & 84.89 $\pm$ 3.00 & 68.89 $\pm$ 1.10 & 88.32 $\pm$ 0.99 & \underline{90.45 $\pm$ 0.14} & 75.74 $\pm$ 0.72 & 84.38 $\pm$ 0.21 & \textbf{93.33 $\pm$ 0.13} & \first{95.95 $\pm$ 0.31} \\
                       & Social Evo. & 92.05 $\pm$ 0.46 & 90.76 $\pm$ 0.21 & 94.76 $\pm$ 0.16 & \underline{95.39 $\pm$ 0.17} & 87.34 $\pm$ 0.08 & 94.84 $\pm$ 0.17 & 95.23 $\pm$ 0.07 & \textbf{96.30 $\pm$ 0.01} & 93.76 $\pm$ 0.63                 \\
                       & UCI         & 90.44 $\pm$ 0.49 & 68.77 $\pm$ 2.34 & 78.53 $\pm$ 0.74 & 92.03 $\pm$ 1.13 & \underline{93.87 $\pm$ 0.08} & 87.82 $\pm$ 1.36 & 91.81 $\pm$ 0.67 & \textbf{94.49 $\pm$ 0.26} & \first{97.89 $\pm$ 0.10} \\
                       & Flights     & 96.21 $\pm$ 1.42 & 95.95 $\pm$ 0.62 & 94.13 $\pm$ 0.17 & 98.22 $\pm$ 0.13 & \underline{98.45 $\pm$ 0.01} & 91.21 $\pm$ 0.02 & 91.13 $\pm$ 0.01 & \textbf{98.93 $\pm$ 0.01} &  99.43 $\pm$ 0.06                \\
                       & Can. Parl.  & 78.21 $\pm$ 0.23 & 73.35 $\pm$ 3.67 & 75.69 $\pm$ 0.78 & 76.99 $\pm$ 1.80 & 75.70 $\pm$ 3.27 & 72.46 $\pm$ 3.23 & \underline{83.17 $\pm$ 0.53} & \textbf{97.76 $\pm$ 0.41} & \first{99.03 $\pm$ 0.03}  \\
                       & US Legis.   & \underline{82.85 $\pm$ 1.07} & 82.28 $\pm$ 0.32 & 75.84 $\pm$ 1.99 & \textbf{83.34 $\pm$ 0.43} & 77.16 $\pm$ 0.39 & 76.27 $\pm$ 0.63 & 76.96 $\pm$ 0.79 & 77.90 $\pm$ 0.58 & \first{84.36 $\pm$ 0.20} \\
                       & UN Trade    & \underline{69.62 $\pm$ 0.44} & 67.44 $\pm$ 0.83 & 64.01 $\pm$ 0.12 & 69.10 $\pm$ 1.67 & 68.54 $\pm$ 0.18 & 64.72 $\pm$ 0.05 & 65.52 $\pm$ 0.51 & \textbf{70.20 $\pm$ 1.44} & \first{77.81 $\pm$ 1.78} \\
                       & UN Vote     & \underline{68.53 $\pm$ 0.95} & 67.18 $\pm$ 1.04 & 52.83 $\pm$ 1.12 & \textbf{69.71 $\pm$ 2.65} & 53.09 $\pm$ 0.22 & 51.88 $\pm$ 0.36 & 52.46 $\pm$ 0.27 & 57.12 $\pm$ 0.62 & \first{76.67 $\pm$ 0.09}  \\
                       & Contact     & 96.66 $\pm$ 0.89 & 96.48 $\pm$ 0.14 & 96.95 $\pm$ 0.08 & \underline{97.54 $\pm$ 0.35} & 89.99 $\pm$ 0.34 & 94.15 $\pm$ 0.09 & 93.94 $\pm$ 0.02 & \textbf{98.53 $\pm$ 0.01} & 98.40 $\pm$ 0.03 \\ \cline{2-11} 
                       & Avg. Rank   & 4.38         & 5.77         & 6.00         & \underline{2.54}         & 4.38         & 7.23         & 5.77         & \textbf{1.62}         &  \\ \hline
\multirow{14}{*}{hist} & Wikipedia   & 80.77 $\pm$ 0.73 & 77.74 $\pm$ 0.33 & 82.87 $\pm$ 0.22 & 82.74 $\pm$ 0.32 & 67.84 $\pm$ 0.64 & \underline{85.76 $\pm$ 0.46} & \textbf{87.68 $\pm$ 0.17} & 78.80 $\pm$ 1.95 & 98.11 $\pm$ 0.04 \\
                       & Reddit      & 80.52 $\pm$ 0.32 & 80.15 $\pm$ 0.18 & 79.33 $\pm$ 0.16 & \textbf{81.11 $\pm$ 0.19} & 80.27 $\pm$ 0.30 & 76.49 $\pm$ 0.16 & 77.80 $\pm$ 0.12 & \underline{80.54 $\pm$ 0.29} &  \\
                       & MOOC        & 82.75 $\pm$ 0.83 & 81.06 $\pm$ 0.94 & 80.81 $\pm$ 0.67 & \textbf{88.00 $\pm$ 1.80} & 71.57 $\pm$ 1.07 & 72.09 $\pm$ 0.56 & 76.68 $\pm$ 1.40 & \underline{87.04 $\pm$ 0.35} &  \\
                       & LastFM      & 75.22 $\pm$ 2.36 & 74.65 $\pm$ 1.98 & 64.27 $\pm$ 0.26 & 77.97 $\pm$ 3.04 & 67.88 $\pm$ 0.24 & 47.24 $\pm$ 3.13 & 64.21 $\pm$ 0.73 & \textbf{78.78 $\pm$ 0.35} & 94.61 $\pm$ 0.62 \\
                       & Enron       & 75.39 $\pm$ 2.37 & 74.69 $\pm$ 3.55 & 61.85 $\pm$ 1.43 & \underline{77.09 $\pm$ 2.22} & 65.10 $\pm$ 0.34 & 67.95 $\pm$ 0.88 & 75.27 $\pm$ 1.14 & 76.55 $\pm$ 0.52 &  \\
                       & Social Evo. & 90.06 $\pm$ 3.15 & 93.12 $\pm$ 0.34 & 93.08 $\pm$ 0.59 & \underline{94.71 $\pm$ 0.53} & 87.43 $\pm$ 0.15 & 93.44 $\pm$ 0.68 & 94.39 $\pm$ 0.31 & \textbf{97.28 $\pm$ 0.07} &  \\
                       & UCI         & \textbf{78.64 $\pm$ 3.50} & 57.91 $\pm$ 3.12 & 58.89 $\pm$ 1.57 & 77.25 $\pm$ 2.68 & 57.86 $\pm$ 0.15 & 72.25 $\pm$ 3.46 & \underline{77.54 $\pm$ 2.02} & 76.97 $\pm$ 0.24 & 95.40 $\pm$ 0.16 \\
                       & Flights     & 68.97 $\pm$ 1.87 & 69.43 $\pm$ 0.90 & \underline{72.20 $\pm$ 0.16} & 68.39 $\pm$ 0.95 & 66.11 $\pm$ 0.71 & 70.57 $\pm$ 0.18 & 70.37 $\pm$ 0.23 & 68.09 $\pm$ 0.43 &                           \\
                       & Can. Parl.  & 62.44 $\pm$ 1.11 & 70.16 $\pm$ 1.70 & 70.86 $\pm$ 0.94 & 73.23 $\pm$ 3.08 & 72.06 $\pm$ 3.94 & 69.95 $\pm$ 3.70 & \underline{79.03 $\pm$ 1.01} & \textbf{97.61 $\pm$ 0.40} & 93.72 $\pm$ 1.33 \\
                       & US Legis.   & 67.47 $\pm$ 6.40 & \textbf{91.44 $\pm$ 1.18} & 73.47 $\pm$ 5.25 & 83.53 $\pm$ 4.53 & 78.62 $\pm$ 7.46 & 83.97 $\pm$ 3.71 & 85.17 $\pm$ 0.70 & \underline{90.77 $\pm$ 1.96} & 88.24 $\pm$ 0.83 \\
                       & UN Trade    & 68.92 $\pm$ 1.40 & 64.36 $\pm$ 1.40 & 60.37 $\pm$ 0.68 & 63.93 $\pm$ 5.41 & 63.09 $\pm$ 0.74 & 61.43 $\pm$ 1.04 & 63.20 $\pm$ 1.54 & \underline{73.86 $\pm$ 1.13} & 84.96 $\pm$ 0.97 \\
                       & UN Vote     & \underline{76.84 $\pm$ 1.01} & 74.72 $\pm$ 1.43 & 53.95 $\pm$ 3.15 & 73.40 $\pm$ 5.20 & 51.27 $\pm$ 0.33 & 52.29 $\pm$ 2.39 & 52.61 $\pm$ 1.44 & 64.27 $\pm$ 1.78 & 81.64 $\pm$ 0.16 \\
                       & Contact     & \underline{96.35 $\pm$ 0.92} & 96.00 $\pm$ 0.23 & 95.39 $\pm$ 0.43 & 93.76 $\pm$ 1.29 & 83.06 $\pm$ 0.32 & 93.34 $\pm$ 0.19 & 93.14 $\pm$ 0.34 & \textbf{97.17 $\pm$ 0.05} &  \\ \cline{2-11} 
                       & Avg. Rank   & 4.38         & 4.77         & 5.85         & \underline{3.46}         & 7.38         & 6.08         & 4.77         & \textbf{2.92}         &  \\ \hline
\multirow{14}{*}{ind}  & Wikipedia   & 70.96 $\pm$ 0.78 & 67.36 $\pm$ 0.96 & 81.93 $\pm$ 0.22 & 80.97 $\pm$ 0.31 & 70.95 $\pm$ 0.95 & \underline{82.19 $\pm$ 0.48} & \textbf{84.28 $\pm$ 0.30} & 75.09 $\pm$ 3.70 & 95.84 ± 01.5 \\
                       & Reddit      & 83.51 $\pm$ 0.15 & 82.90 $\pm$ 0.31 & \underline{87.13 $\pm$ 0.20} & 84.56 $\pm$ 0.24 & \textbf{88.04 $\pm$ 0.29} & 84.67 $\pm$ 0.29 & 82.21 $\pm$ 0.13 & 86.23 $\pm$ 0.51 &  \\
                       & MOOC        & 66.63 $\pm$ 2.30 & 63.26 $\pm$ 1.01 & 73.18 $\pm$ 0.33 & \underline{77.44 $\pm$ 2.86} & 70.32 $\pm$ 1.43 & 70.36 $\pm$ 0.37 & 72.45 $\pm$ 0.72 & \textbf{80.76 $\pm$ 0.76} &  \\
                       & LastFM      & 61.32 $\pm$ 3.49 & 62.15 $\pm$ 2.12 & 63.99 $\pm$ 0.21 & 65.46 $\pm$ 4.27 & 67.92 $\pm$ 0.44 & 46.93 $\pm$ 2.59 & 60.22 $\pm$ 0.32 & \underline{69.25 $\pm$ 0.36} & 93.28 $\pm$ 0.71 \\
                       & Enron       & 70.92 $\pm$ 1.05 & 68.73 $\pm$ 1.34 & 60.45 $\pm$ 2.12 & 71.34 $\pm$ 2.46 & \textbf{75.17 $\pm$ 0.50} & 67.64 $\pm$ 0.86 & 71.53 $\pm$ 0.85 & 74.07 $\pm$ 0.64 &  \\
                       & Social Evo. & 90.01 $\pm$ 3.19 & 93.07 $\pm$ 0.38 & 92.94 $\pm$ 0.61 & \underline{95.24 $\pm$ 0.56} & 89.93 $\pm$ 0.15 & 93.44 $\pm$ 0.72 & 94.22 $\pm$ 0.32 & \textbf{97.51 $\pm$ 0.06} &  \\
                       & UCI         & 64.14 $\pm$ 1.26 & 54.25 $\pm$ 2.01 & 60.80 $\pm$ 1.01 & 64.11 $\pm$ 1.04 & 58.06 $\pm$ 0.26 & \underline{70.05 $\pm$ 1.86} & \textbf{74.59 $\pm$ 0.74} & 65.96 $\pm$ 1.18 & 87.51 $\pm$ 0.25 \\
                       & Flights     & 69.99 $\pm$ 3.10 & 71.13 $\pm$ 1.55 & \underline{73.47 $\pm$ 0.18} & 71.63 $\pm$ 1.72 & 69.70 $\pm$ 0.75 & 72.54 $\pm$ 0.19 & 72.21 $\pm$ 0.21 & 69.53 $\pm$ 1.17 &                           \\
                       & Can. Parl.  & 52.88 $\pm$ 0.80 & 63.53 $\pm$ 0.65 & 72.47 $\pm$ 1.18 & 69.57 $\pm$ 2.81 & \underline{72.93 $\pm$ 1.78} & 69.47 $\pm$ 2.12 & 70.52 $\pm$ 0.94 & \textbf{96.70 $\pm$ 0.59} & 87.68 $\pm$ 2.16 \\
                       & US Legis.   & 59.05 $\pm$ 5.52 & \textbf{89.44 $\pm$ 0.71} & 71.62 $\pm$ 5.42 & 78.12 $\pm$ 4.46 & 76.45 $\pm$ 7.02 & 82.54 $\pm$ 3.91 & 84.22 $\pm$ 0.91 & \underline{87.96 $\pm$ 1.80} & 84.65 $\pm$ 0.17 \\
                       & UN Trade    & 66.82 $\pm$ 1.27 & 65.60 $\pm$ 1.28 & 66.13 $\pm$ 0.78 & 66.37 $\pm$ 5.39 & \underline{71.73 $\pm$ 0.74} & 67.80 $\pm$ 1.21 & 66.53 $\pm$ 1.22 & 62.56 $\pm$ 1.51 & 84.39 ± 0.91 \\
                       & UN Vote     & \textbf{73.73 $\pm$ 1.61} & 72.80 $\pm$ 2.16 & 53.04 $\pm$ 2.58 & 72.69 $\pm$ 3.72 & 52.75 $\pm$ 0.90 & 52.02 $\pm$ 1.64 & 51.89 $\pm$ 0.74 & 53.37 $\pm$ 1.26 & 78.92 $\pm$ 0.18 \\
                       & Contact     & \underline{94.47 $\pm$ 1.08} & 94.23 $\pm$ 0.18 & 94.10 $\pm$ 0.41 & 91.64 $\pm$ 1.72 & 87.68 $\pm$ 0.24 & 91.23 $\pm$ 0.19 & 90.96 $\pm$ 0.27 & \textbf{95.01 $\pm$ 0.15} &  \\ \cline{2-11} 
                       & Avg. Rank   & 5.92         & 6.15         & 4.85         & \underline{4.54}         & 5.15         & 5.00         & 4.77         & \textbf{3.54}         &  \\ \hline

\end{tabular}
}
}
\label{tab:auc_roc_transductive_dynamic_link_prediction}
\end{table}

==> tables/runtime_simpletlp.tex <==
\begin{table}[h]
\centering
\caption{Runtime (in seconds) and number of training epochs of SimpleTLP for each datasets across 5 runs}
\begin{tabular}{c&c&c}
\hline
Dataset & Total Time for 5 runs (in seconds) & Number of Training Epochs for 5 runs \\ 
\hline
Wikipedia & [20491.54, 19836.15, 25806.94,14049.88, 13747.04] & [53, 55, 72, 38, 38] \\
Reddit & [90828.53 , 54464.69 , 66810.79 , 79976.49 , 34474.04 ] & [44, 30, 34, 41, 25] \\
MOOC  & [29130.86, 34566.03, 47800.52, 26011.17, 52037.48] & [32, 41, 54, 30, 61] \\
LastFM & [31555.95, 27008.17, 41525.32, 27177.40, 26147.18] & [28, 25, 39, 27, 26] \\
Enron & [2299.42 , 3403.21 , 3578.98 , 1955.66 , 2879.50 ] & [21, 37, 39, 21, 32] \\
SocialEvo & [55329.37 , 67586.07 , 16118.38 , 84248.00 , 62308.54 ] & [38, 47, 30, 73, 39] \\
UCI & [4490.47 , 1908.67 , 3029.95 , 1801.28 , 3512.28 ] & [38, 17, 27, 16, 35] \\
Flights & [81917.03 , 119708.01 , 75354.95 , 163200.20, 70091.67 ] & [12, 19, 11, 27, 15] \\
Can. Parl. & [818.45 , 896.20 , 1531.42 , 1636.52 , 1532.19 ] & [19, 20, 31, 35, 37] \\
US Legis. & [287.19 , 257.18 , 251.49 , 248.92 , 305.09 ] & [21, 18, 17, 17, 21] \\
UN Trade. & [2922.14 ,2857.13 , 2450.84 , 2593.40 , 2740.26 ] & [21, 21, 18, 18, 19] \\
UN Vote & [2424.91 , 2445.20 , 3388.58 , 2454.06 , 2430.62 ] & [12, 12, 17, 12, 12] \\
Contact & [72622.20 , 54611.65 , 52249.71 , 114934.51 , 67422.84] & [38, 30, 33, 59, 52] \\ 
\hline
\end{tabular}
\label{tab:runtime_simpletlp}
\end{table}
